Pure Spectral Graph Embeddings: Reinterpreting Graph Convolution for Top-N Recommendation

The use of graph convolution in the development of recommender system algorithms has recently achieved state-of-the-art results in the collaborative filtering task (CF). While it has been demonstrated that the graph convolution operation is connected to a filtering operation on the graph spectral domain, the theoretical rationale for why this leads to higher performance on the collaborative filtering problem remains unknown. The presented work makes two contributions. First, we investigate the effect of using graph convolution throughout the user and item representation learning processes, demonstrating how the latent features learned are pushed from the filtering operation into the subspace spanned by the eigenvectors associated with the highest eigenvalues of the normalised adjacency matrix, and how vectors lying on this subspace are the optimal solutions for an objective function related to the sum of the prediction function over the training data. Then, we present an approach that directly leverages the eigenvectors to emulate the solution obtained through graph convolution, eliminating the requirement for a time-consuming gradient descent training procedure while also delivering higher performance on three real-world datasets.

==> tex_figures/ablation_alpha.tex <==
\begin{figure*}
    \centering
    \subfloat[]{\includegraphics[width=0.5\textwidth, keepaspectratio]{main/images/Movielens1M_alpha_item_pop.pdf}}
    \subfloat[]{\includegraphics[width=0.5\textwidth, keepaspectratio]{main/images/Movielens1M_alpha_user_length.pdf}}
    \caption{caption}
    \label{fig:ablation_alpha}
\end{figure*}

==> tex_figures/ablation_k.tex <==
\begin{figure*}
    %\vskip 0.1in
    \centering
    \subfigure[Movielens1M]{\includegraphics[width=0.32\columnwidth]{images/Movielens1M_sp_perf2.pdf}}
    \subfigure[Amazon]{\includegraphics[width=0.32\columnwidth]{images/Amazon Electronics_sp_perf2.pdf}}
    \subfigure[Gowalla]{\includegraphics[width=0.32\columnwidth]{images/Gowalla_sp_perf2.pdf}}
    \caption{PSGE performance varying the amount of the top-$k$ eigenvectors used to construct the embeddings. On the right $y$-axis is reported the eigenvalue related to the eigenvector added, while the number of eigenvectors used to construct the user and item embeddings is reported on the $x$-axis. The dotted blue line indicates the $k$ associated to the best performance.}
    %\vskip -0.2in
    \label{fig:ablation_k}
\end{figure*}



==> tex_figures/effect_convolution.tex <==
\begin{figure}
    %\vskip 0.1in
    \centering
    \subfigure[]{\includegraphics[width=0.33\columnwidth]{images/span_corr_through_epoch.pdf}\label{subfig:conv_learning}}
    \subfigure[]{\includegraphics[width=0.33\columnwidth]{images/progressive_span.pdf}\label{subfig:conv_convergence}}
    \caption{Figure (a) shows the extent to which the latent features learned from BPR and LightGCN, are contained in the subspace spanned by the first $\ell=20$ eigenvectors. Figure (b) shows the cumulative correlation of the signals learned at convergence from BPR and LightGCN.}
    %\vskip -0.2in
    \label{fig:effect_convolution}
\end{figure}

==> tex_figures/progressive_span.tex <==
\begin{figure}
    %\vskip 0.1in
    \begin{center}
    \centerline{\includegraphics[width=1\columnwidth]{images/colwidth_span_corr_through_epoch.pdf}}
    \caption{$\rho(\mathrm{X})$ varying $\ell$ for LightGCN and BPR}
    \label{fig:convergence_span_corr}
    \end{center}
    \vskip -0.2in
\end{figure}

==> tex_figures/rel_avg_popularity_exp.tex <==
\begin{figure*}
    \centering
    \subfloat[Movielens1M]{\includegraphics[width=0.33\columnwidth, keepaspectratio]{main/images/Movielens1M_Relative Average Popularity.pdf}}
    \subfloat[Amazon]{\includegraphics[width=0.33\columnwidth, keepaspectratio]{main/images/AmazonElectronics_Relative Average Popularity.pdf}}
    \subfloat[Gowalla]{\includegraphics[width=0.33\columnwidth, keepaspectratio]{main/images/Gowalla_Relative Average Popularity.pdf}}
    \caption{Relative Average Popularity}
    \label{fig:pop-exp}
\end{figure*}



==> tex_figures/span_corr_through_epoch.tex <==
\begin{figure}
    %\vskip 0.1in
    \begin{center}
    \centerline{\includegraphics[width=1\columnwidth]{images/colwidth_span_corr_through_epoch.pdf}}
    \caption{$\rho(\mathrm{X})$ vs epoch for embeddings learned on ML1m dataset, with $\ell=20$. }
    \label{fig:span_corr_through_epoch}
    \end{center}
    %\vskip -0.2in
\end{figure}

==> tex_figures/span_exp.tex <==
\begin{figure}[]
    \vskip 0.2in
    \centering
    \subfloat[caption]{\includegraphics[width=0.49\columnwidth]{main/images/v_span_corr_through_epoch.pdf}}
    \subfloat[caption]{\includegraphics[width=0.49\columnwidth]{main/images/v_progressive_span.pdf}}
    %\vskip -0.2in
    \caption{aa}
\end{figure}

==> tex_tables/dataset_stat.tex <==
\begin{table}[ht]
\caption{Datasets statistics, we report the number of user item interactions and density of the preprocessed datasets.}
\label{table:dataset_stat}
%\vskip 0.15in
\begin{center}
\small
\setlength{\tabcolsep}{4pt}
\begin{sc}
\begin{tabular}{lrrrr}
\toprule
Dataset & User & Item & Interactions & Density \\
\midrule
ML1M& 5 949& 2 810& 571 531&3.4 $10^{-2}$\\
Amazon    & 9 279& 6 065& 158 979&2.8 $10^{-3}$\\
Gowalla    & 29 858& 40 988& 1 027 464&8.4 $10^{-4}$\\
\bottomrule
\end{tabular}
\end{sc}

\end{center}
\vskip -0.1in
\end{table}

==> tex_tables/performance_table.tex <==
\begin{table*}[!t]
\caption{Recommendation performance comparison. Bold and underline indicate best and second best performing algorithm.}
\vskip 0.15in
\small
\setlength{\tabcolsep}{5pt}
\centering
\begin{tabular}{ccccc@{\hspace{10pt}}cccc@{\hspace{10pt}}cccc@{\hspace{10pt}}cccc}
\toprule 

\multirow{3}{*}{Model} &

\multicolumn{4}{c}{\textbf{Ml1M}} &
\multicolumn{4}{c}{\textbf{Amazon}} &
\multicolumn{4}{c}{\textbf{Gowalla}} \\

% horizontal line under dataset name
\cmidrule(l{15pt}r{20pt}){2-5}
\cmidrule(l{15pt}r{20pt}){6-9}
\cmidrule(l{15pt}r{20pt}){10-13}
& 
 \multicolumn{2}{c}{NDCG} & 
 \multicolumn{2}{c}{Recall} &
 
 \multicolumn{2}{c}{NDCG} & 
 \multicolumn{2}{c}{Recall} &
 
 \multicolumn{2}{c}{NDCG} &
 \multicolumn{2}{c}{Recall}  \\ 
 
 & 
 @5 & @20 & @5 & @20 & 
 @5 & @20 & @5 & @20 & 
 @5 & @20 & @5 & @20 \\ \midrule
 
 BPR-MF &
 % Movielens1m
 0.1270 & 0.2203 & 0.1028 & 0.2521  & 
 % Amazon
 0.0232 & 0.0397 & 0.0318 & 0.0854  &
 % Gowalla
 0.0625 & 0.0966 & 0.0725 & 0.1643\\
 
  LightGCN &
 % Movielens1m
 0.1311 & 0.2272 & 0.1079 & 0.2660  & 
 % Amazon
 0.0245 & 0.0424 & 0.0337 & 0.0911  &
 % Gowalla
 0.0810 & 0.1179 & 0.0905 & 0.1948\\
 
 EASE &
 % Movielens1m
 \textbf{0.1473} & \underline{0.2469} & \underline{0.1194} & 0.2816  & 
 % Amazon
 \underline{0.0284} & 
 0.0463 & 0.0378 & 0.0952  &
 % Gowalla
 0.0885 & \underline{0.1335} & 0.1008 & \underline{0.2191}\\
 
  SGMC &
 % Movielens1m
 0.1397 & 0.2406 & 0.1145 & \underline{0.2832}  & 
 % Amazon
 0.0286 & \textbf{0.0471} & \textbf{0.0398} & \textbf{0.0990}  & 
 % Gowalla
 \underline{0.0895} & 0.1332 & \underline{0.1017} & 0.2157  \\
 
 \midrule
    PSGE &
% Movielens1m
 0.1294 & 0.2241 & 0.1067 & 0.2682  & 
 % Amazon
 0.0279 & 0.0452 & 0.0384 & 0.0946  & 
 % Gowalla
 0.0864 & 0.1281 & 0.0972 & 0.2059  \\
    
    PSIS &
% Movielens1m
 0.1358 & 0.2381 & 0.1131 & 0.2824  & 
 % Amazon
 0.0272 & 0.0448 & 0.0376 & 0.0946  & 
 % Gowalla
 0.0862 & 0.1296 & 0.0977 & 0.2124  \\
     
     PSUS &
% Movielens1m
 \underline{0.1457} & \textbf{0.2483} & \textbf{0.1195} & \textbf{0.2915}  & 
 % Amazon
 \textbf{0.0287} & \underline{0.0470} & \underline{0.0394} & \underline{0.0989}  & 
 % Gowalla
 \textbf{0.0920} & \textbf{0.1368} & \textbf{0.1048} & \textbf{0.2217}  \\

\midrule
      PSGE++ &
 %Movielens1m
  - & - & - & - &
  %Amazon
  - & - & - & - &
  %Gowalla
 - & - & - & - \\

      SGE &
% Movielens1m
 0.1397 & 0.2419 & 0.1138 & 0.2833 & 
 % Amazon
 0.0282 & 0.0466 & 0.0394 & 0.0987& 
 % Gowalla
% - & - & - & - \\

\bottomrule
\end{tabular}
\label{table:performance_table}
\end{table*}

==> tex_tables/size_time_table.tex <==
\begin{table}[!t]
\caption{Effect on PSGE and LighGCN of the embedding size on the performance and training time.}
%\vskip 0.15in
\small
\setlength{\tabcolsep}{3pt}
\centering
\begin{tabular}{cllrrlrl@{\hspace{10pt}}}
\toprule 

%\multirow{2}{*}{\textbf{Dataset}} &
\multirow{2}{*}{} &
\multirow{2}{*}{\textbf{Model}} &
\multirow{2}{*}{\textbf{Size}} &
\multirow{2}{*}{\textbf{Tr Time}} &


 
 \multicolumn{2}{c}{\textbf{NDCG}} &
 \multicolumn{2}{c}{\textbf{Recall}}  \\ 
 
 &&&&@5 & @20 & @5 & @20 \\ \midrule
 
 \multirow{3}{*}[-2pt]{\begin{turn}{90}\textbf{Ml1M}\end{turn}} 
 %\multirow{3}{*}[-2pt]{\textbf{Ml1M}} 
 &\multirow{2}{*}{LGCN} 
 % Movielens1m 64
 &64 & 24m 45s & 0.1647 & 0.2679 & 0.1254 & 0.2898  \\
 % Movielens1m 80
 &&80 & 48m 18s & 0.1648 & 0.2680 & 0.1254 & 0.2904  \\
\cmidrule{2-8}
 &PSGE & 80 & 8s & \textbf{0.1839} & \textbf{0.2951} & \textbf{0.1418} & \textbf{0.3230} \\
 \midrule
 
 %\multirow{3}{*}[-2pt]{\textbf{Amazon}} 
 \multirow{3}{*}[-2pt]{\begin{turn}{90}\textbf{Amazon}\end{turn}} 
 
 &\multirow{2}{*}{LGCN} 
 % Movielens1m 64
 &64 & 5m 54s & 0.0261 &0.0446& 0.0357& 0.0956  \\
 % Movielens1m 80
 &&80 & 6m 23s & 0.0262 & 0.0447 & 0.0356 & 0.0956  \\
\cmidrule{2-8}
 &PSGE & 80 & 10s & \textbf{0.0339} & \textbf{0.0533} & \textbf{0.0458} & \textbf{0.1087} \\ 
 \midrule
 
%  \textbf{0.0339} & \textbf{0.0533} & \textbf{0.0458} & \textbf{0.1087} \\ 
 
 %\multirow{4}{*}[-2pt]{\textbf{Gowalla}} 
 \multirow{4}{*}[-2pt]{\begin{turn}{90}\textbf{Gowalla}\end{turn}} 
  &\multirow{3}{*}{LGCN} 
 % Gowalla 64
%  &64 & 2h 38m 18s & 0.0873 &0.1277 &0.0980 & 0.2050  \\
 &64 & 2h 38m& 0.0873 &0.1277 &0.0980 & 0.2050  \\
 % Gowalla 512
%  &&512 & 21h 06m 17s & 0.0957 & 0.1386 & 0.1073 & 0.2206  \\
 &&512 & 21h 06m & 0.0957 & 0.1386 & 0.1073 & 0.2206  \\
 % Gowalla 1024
%  &&1024 & 49h 17m 09s& 0.0957 & 0.1384 & 0.1071 & 0.2196  \\
&&1024 & 49h 17m& 0.0957 & 0.1384 & 0.1071 & 0.2196  \\
 \cmidrule{2-8}
 
 &PSGE & 1500 & 39m 28s & \textbf{0.1155} & \textbf{0.1641} & \textbf{0.1265} & \textbf{0.2519}\\
 
%   PSGE &
% % Movielens1m % beta=0.3 aloha=0.4 k=80
%  \underline{0.1839} & \underline{0.2951} & \textbf{0.1418} & \textbf{0.3230} &
%  % Amazon k=80 alpha=0.5, beta=0.3
%  \textbf{0.0339} & \textbf{0.0533} & \textbf{0.0458} & \textbf{0.1087} & 
%  % Gowalla alpha=0.4, beta=0.3 
% %  \textbf{0.1117} & \textbf{0.1605} & \textbf{0.1218} & \textbf{0.2477}\\
% \textbf{0.1155} & \textbf{0.1641} & \textbf{0.1265} & \textbf{0.2519}\\
 
 % Gowalla
 %0.0873 & 0.1277 & 0.0980 & 0.2050  \\
 
%  LightGCN 64&
%  % Amazon
%  0.0261 & 0.0446 & 0.0357 & 0.0956  \\
 
\bottomrule
\end{tabular}
\label{table:training_time}
\end{table}

==> tex_tables/trainval_perf_table.tex <==
\begin{table*}[!t]
\caption{Recommendation performance. bold and underline indicate the first and the second best performing algorithms.}
%\vskip 0.15in
% \small
\setlength{\tabcolsep}{1pt}
\centering
\begin{tabular}{l@{\hspace{10pt}}cccc@{\hspace{10pt}}cccc@{\hspace{10pt}}cccc}
\toprule 

\multirow{3}{*}{\textbf{Model}} &

\multicolumn{4}{c}{\textbf{Ml1M}} &
\multicolumn{4}{c}{\textbf{Amazon}} &
\multicolumn{4}{c}{\textbf{Gowalla}} \\

% horizontal line under dataset name
\cmidrule(l{15pt}r{20pt}){2-5}
\cmidrule(l{15pt}r{20pt}){6-9}
\cmidrule(l{15pt}r{20pt}){10-13}
& 
 \multicolumn{2}{c}{NDCG} & 
 \multicolumn{2}{c}{Recall} &
 
 \multicolumn{2}{c}{NDCG} & 
 \multicolumn{2}{c}{Recall} &
 
 \multicolumn{2}{c}{NDCG} &
 \multicolumn{2}{c}{Recall}  \\ 
 
 & 
 @5 & @20 & @5 & @20 & 
 @5 & @20 & @5 & @20 & 
 @5 & @20 & @5 & @20 \\ \midrule
 
 BPR-MF &
 % Movielens1m
 0.1600 & 0.2602 & 0.1191 & 0.2756  &
 % Amazon
 0.0269 & 0.0439 & 0.0377 & 0.0928  & 
 % Gowalla
 0.0665 & 0.1021 & 0.0763 & 0.1721  \\
 
  LightGCN &
 % Movielens1m
 0.1647 & 0.2679 & 0.1254 & 0.2898  &
 % Amazon
 0.0261 & 0.0446 & 0.0357 & 0.0956  & 
 % Gowalla
 0.0873 & 0.1277 & 0.0980 & 0.2050  \\
 
 \midrule
 
     PureSVD &
% Movielens1m
 0.1623 & 0.2621 & 0.1203 & 0.2755  & 
 % Amazon
 0.0160 & 0.0299 & 0.0229 & 0.0682  & 
 % Gowalla
 0.0789 & 0.1162 & 0.0860 & 0.1836  \\
 
 EASE &
 % Movielens1m
 \textbf{0.1866} & \textbf{0.2969} & \underline{0.1415} & \underline{0.3164}  & 
 % Amazon
 0.0325 & 0.0509 & 0.0435 & 0.1028  & 
 % Gowalla
 0.1008 & 0.1469 & 0.1114 & 0.2319 \\
 
  SGMC &
 % Movielens1m
 0.1765 & 0.2830 & 0.1369 & 0.3070  & 
 % Amazon
 \underline{0.0330} & \underline{0.0528} & \underline{0.0443} & \textbf{0.1087}  & 
 % Gowalla
 \underline{0.1023} & \underline{0.1514} & \underline{0.1167} & \underline{0.2328}  \\
 
 \midrule

 %   PSGE_old &
% Movielens1m
% 0.1599 & 0.2592 & 0.1263 & 0.2896  & 
 % Amazon
% 0.0301 & 0.0490 & 0.0413 & 0.1020  & 
 % Gowalla
% 0.0998 & 0.1427 & 0.1100 & 0.2205  \\
    
%    PSIS &
% Movielens1m
% 0.1756 & 0.2871 & 0.1313 & 0.3106  & 
 % Amazon
% 0.0311 & 0.0501 & 0.0430 & 0.1053  & 
 % Gowalla
% 0.0986 & 0.1429 & 0.1089 & 0.2256  \\
     
%    PSUS &
% Movielens1m
% 0.1853 & 0.2935 & 0.1416 & 0.3140 & 
 % Amazon
% 0.0338 & 0.0529 & 0.0457 & 0.1078& 
 % Gowalla
% 0.1047 & 0.1505 & 0.1160 & 0.2352  \\
      
%       PSGE-$\lambda^2$ &
% % Movielens1m
%  \underline{0.1863} & \underline{0.2958} & \textbf{0.1435} & \textbf{0.3194} & 
%  % Amazon
%  \textbf{0.0340} & \textbf{0.0539} & \textbf{0.0473} & \textbf{0.1113}& 
%  % Gowalla
%  \textbf{0.1079} & \textbf{0.1571} & \textbf{0.1172} & \textbf{0.2445} \\ 
 
%       PSGE-$\lambda$ &
% % Movielens1m
%  0.1713 & 0.2760 & 0.1344 & 0.3036 & 
%  % Amazon
%  - & - & - & -& 
%  % Gowalla
%  - & - & - & -\\
 
%         PSGE-$\lambda \mat{D}_i^\alpha$ &
% % Movielens1m
%  0.1834 & 0.2924 & 0.1421 & 0.3210 & 
%  % Amazon
%  \underline{0.0330} & \underline{0.0528} & \underline{0.0443} & \underline{0.1087}  & 
%  % Gowalla
%  0.1043 & 0.1511 & 0.1147 & 0.2358\\
 
% PSGE &
% % Movielens1m
%  - & - & - & - &
%  % Amazon
%  - & - & - & - &
%  % Gowalla
%  - & - & - & - \\
 
%  PSGE+ &
% % Movielens1m
%  - & - & - & - &
%  % Amazon
%  - & - & - & - &
%  % Gowalla
%  - & - & - & - \\
 
 
 PSGE &
% Movielens1m % beta=0.3 aloha=0.4 k=80
 \underline{0.1839} & \underline{0.2951} & \textbf{0.1418} & \textbf{0.3230} &
 % Amazon k=80 alpha=0.5, beta=0.3
 \textbf{0.0339} & \textbf{0.0533} & \textbf{0.0458} & \textbf{0.1087} & 
 % Gowalla alpha=0.4, beta=0.3 
%  \textbf{0.1117} & \textbf{0.1605} & \textbf{0.1218} & \textbf{0.2477}\\
\textbf{0.1155} & \textbf{0.1641} & \textbf{0.1265} & \textbf{0.2519}\\
 
% \midrule
% $\alpha$-EASE &
% % Movielens1m
%  \textbf{0.1889} & \textbf{0.3006} & \textbf{0.1442} & \textbf{0.3225} & 
%  % Amazon
% \textbf{0.0383} & \textbf{0.0577} & \textbf{0.0508} & \textbf{0.1125}  & 
%  % Gowalla
%  - & - & - & -\\



\bottomrule
\end{tabular}
\label{table:performance_table}
\end{table*}
